A machine learning approach to mapping baryons onto dark matter haloes using the EAGLE and C-EAGLE simulations

High-resolution cosmological hydrodynamic simulations are currently limited to relatively small volumes due to their computational expense. However, much larger volumes are required to probe rare, overdense environments, and measure clustering statistics of the large scale structure. Typically, zoom simulations of individual regions are used to study rare environments, and semi-analytic models and halo occupation models applied to dark matter only (DMO) simulations are used to study the Universe in the large-volume regime. We propose a new approach, using a machine learning framework to explore the halo-galaxy relationship in the periodic EAGLE simulations, and zoom C-EAGLE simulations of galaxy clusters. We train a tree based machine learning method to predict the baryonic properties of galaxies based on their host dark matter halo properties. The trained model successfully reproduces a number of key distribution functions for an infinitesimal fraction of the computational cost of a full hydrodynamic simulation. By training on both periodic simulations as well as zooms of overdense environments, we learn the bias of galaxy evolution in differing environments. This allows us to apply the trained model to a larger DMO volume than would be possible if we only trained on a periodic simulation. We demonstrate this application using the $(800 \; \mathrm{Mpc})^3$ P-Millennium simulation, and present predictions for key baryonic distribution functions and clustering statistics from the EAGLE model in this large volume.

==> ideas.tex <==

\section{Ideas}

\begin{itemize}

\item{ Page 7 of \cite{reddick_connection_2013} shows common clustering statistics used to evaluate SHAM models. Apply the same to ML model.}

\item{Assembly Bias is the dependence of the clustering of dark matter haloes on properties other than their mass. It provides a tension with HOD models which only use halo mass as a parameter determining halo occupation. Could use ML to quantify assembly bias, and identify the parameters needed to counteract it.}

\item{ Stellar mass / Halo mass relation. \citep{mitchell_evolution_2016} look at evolution of halo-galaxy relation over time. Compare to other models, in particular abundance matching models \citep{behroozi_comprehensive_2010}.}

\item{Directly compare with \cite{simha_testing_2012}, who compare a SHAM with a hydrodynamic simulation. They investigate whether adding a parameter to the SHAM can increase the predictive accuracy. Could present the paper in the same vein.}

\item{\cite{simha_testing_2012} look at luminosity functions in a SHAM, comparing to true SPH values (modelled through SPS). Find greater spread, but still centered on true values.}

\item{\cite{simha_testing_2012} investigate whether SHAM can be used to predict rest frame UV luminosities of high-z galaxies, given that these are dependent on SFR, rather than stellar mass. }

\item{See \cite{weinberg_baryon_2008} for a similar investigation}

\end{itemize}


==> sams.tex <==

\section{Comparing with Semi-Analytic Models}

Figure \ref{fig:eagle_trained_gsmf} shows the galaxy stellar mass function for Henriques2015 and our model. The model successfully reproduces a similar stellar mass function on all scales.

It is important to reiterate that the SAM model and our prediction are completely independent, and that the prediction is based on a very different interpretation of the galaxy physics than the SAM. Any discrepancies between the two can either be attributed to this fundamental difference, or the models failure to reproduce the relationship.


%%%%%%% SAM SMF %%%%%%%%%%

\begin{figure}
	% To include a figure from a file named example.*
	% Allowable file formats are eps or ps if compiling using latex
	% or pdf, png, jpg if compiling using pdflatex
	\includegraphics[width=\columnwidth]{images/gsmf_henriques_fit.png}
    \caption{Galaxy stellar mass function for the matched \eagle\ test set against the predicted stellar mass. Both mass functions are smoothed with a Gaussian of standard deviation 0.1 dex.}
    \label{fig:eagle_trained_gsmf}
\end{figure}

